LEAP nets for power grid perturbations

We propose a novel neural network embedding approach to model power transmission grids, in which high voltage lines are disconnected and reconnected with one-another from time to time, either accidentally or willfully. We call our architeture LEAP net, for Latent Encoding of Atypical Perturbation. Our method implements a form of transfer learning, permitting to train on a few source domains, then generalize to new target domains, without learning on any example of that domain. We evaluate the viability of this technique to rapidly assess cu-rative actions that human operators take in emergency situations, using real historical data, from the French high voltage power grid.

==> glossary.tex <==
\usepackage[xindy,toc]{glossaries}
\renewcommand*{\glstextformat}[1]{\textcolor{black}{#1}}

\makeglossaries
\newglossaryentry{line}
{
  name=transmission line,
  description={is a generic term to denote everything that transmit flow in a power grid. Not to be confused with \gls{conn}}
}
\newglossaryentry{lf}
{
  name=load-flow,
  description={is both a model and an algorithm that allow people to compute the flow on each transmission line in a power grid given the injections. It can alternatively be called power-flow}
}
\newglossaryentry{inj}
{
  name=injection,
  description={is an object that inject (or extract) power from a \gls{grid}. Most often, if the value of power injected is positive we will speak of production. If this value is negative, it will be called a load, or consumption}
}
\newglossaryentry{grid}
{
  name=power grid,
  description={aims at transmitting the power from the production to the consumers. Be careful not to confuse it with \gls{ann} or graph}
}
\newglossaryentry{ann}
{
  name=neural network,
  long=artificial neural network,
  description={is a machine learning model. Be careful not to confuse it with \gls{grid} or graph}
}
\newglossaryentry{graph}
{
  name=graph,
  description={is a representation of a \gls{ann}. Not be confused with \gls{ann} or \gls{grid}}
}
\newglossaryentry{conn}
{
  name=connection,
  description={is weight in an \gls{ann}. Not to be confused with \gls{line}}
}
\newglossaryentry{topo}
{
  name=topology,
  description={corresponds to the way the objects (loads, productions, lines etc.) are connected together in an power-grid. Not to be confused with \gls{arch}}
}
\newglossaryentry{arch}
{
  name=architecture,
  description={applies only to neural networks, and corresponds to the way the connections are organized within. Not to be confused with \gls{topo}}
}
\newglossaryentry{reftopo}
{
  name=reference topology,
  description={topology of the power grid before any lines disconnection TODO}
}
\newglossaryentry{skeleton}
{
  name=underlying skeleton,
  description={complete set of connections TODO}
}
\newglossaryentry{barch}
{
  name=base architecture,
  description={architecture with $\sigma_0$ for reference topology. TODO}
}
\newglossaryentry{mask}
{
  name=mask,
  description={connection pattern TODO}
}
\newglossaryentry{globtopo}
{
  name=global topology,
  description={list/vector of local topologies}
}
\newglossaryentry{loctopo}
{
  name=local topology,
  description={topology of a substation TODO}
}

